DecomCAM: Advancing Beyond Saliency Maps through Decomposition and Integration

Interpreting complex deep networks, notably pre-trained vision-language models (VLMs), is a formidable challenge. Current Class Activation Map (CAM) methods highlight regions revealing the model's decision-making basis but lack clear saliency maps and detailed interpretability. To bridge this gap, we propose DecomCAM, a novel decomposition-and-integration method that distills shared patterns from channel activation maps. Utilizing singular value decomposition, DecomCAM decomposes class-discriminative activation maps into orthogonal sub-saliency maps (OSSMs), which are then integrated together based on their contribution to the target concept. Extensive experiments on six benchmarks reveal that DecomCAM not only excels in locating accuracy but also achieves an optimizing balance between interpretability and computational efficiency. Further analysis unveils that OSSMs correlate with discernible object components, facilitating a granular understanding of the model's reasoning. This positions DecomCAM as a potential tool for fine-grained interpretation of advanced deep learning models. The code is avaible at https://github.com/CapricornGuang/DecomCAM.

==> README.tex <==
DecomCAM: Interpretation via decomposition and open-vocabulary attributes


本论文的核心是什么？我们需要确定我们的优点核心

重点一：
基于GradCAM的，SVD分解+融合 -> 去噪，加速等，这些传统热图的改进。着眼点是，梯度带来的噪声。所以我们需要利用权重，选择梯度大的那些channel。进一步去噪声，我们利用svd分解，把秩小的进一步去掉，只保留主成分。->\textbf{ 重点一，选取重要的channel以及svd，目的都是去噪，需要一点参考文献。}这个是svd本职工作应该好说

为什么融合？ - 需要注意，可以参考scoreCAM？
然后我们根据主成分的权重，进行融合，最终得到我们的目标

这里有一个重点，我需要确认下，我们的融合不是基于channel而是基于主成分的？这点是区分scoreCAM的关键。
\textcolor{blue}{reply: 对的，后面也提供了计算时间来区分}

重点二，
我们svd的分解和融合都是着眼主成分，这种成分本身是一种高层语义？（需要参考文献支持，-> 为什么主成分能和属性这些东西建立联系，跟channel wise的比，核心优点为啥能出来？需要一些SVD、或者分析类解释类的参考文献支持。）因此远远优于基于channel的这种形式？

这也直接造成我们可以对于我们的目标进行一种高层语义级别的分析。这种高层语义在我看来就是所谓的属性一类的。因此我们借助大模型，进一步设计了一种框架。简单有效的把这种可解释，从feature级别的channel level转到高层语义。
\textcolor{blue}{Q:  framework or experiment setting}

非常重要的参考文献
The SVD of Convolutional Weights: A CNN Interpretability Framework. 没有发表只是arxiv，可以不引用。但是参考。
这篇文章写的跟我们异曲同工

""
CNN interpretability literature tends to look to the channel and spatial activations of hidden layer representations to explain the feature maps learned by the model
""


The Singular Values of Convolutional Layers. ICLR2019.
Speeding up Convolutional Neural Networks with Low Rank Expansions
CONVOLUTIONAL NEURAL NETWORKS WITH LOW-RANK REGULARIZATION

Motivation重点

https://ts2.space/zh/ 可解释的人工智能在建立自动驾驶汽车信任中的作/
XAI 是一种人工智能 (AI) 系统，旨在使其决策过程透明且可解释。 通过了解自动驾驶汽车做出决策背后的基本原理，消费者可以深入了解车辆的工作原理，并更有信心信任它。
XAI 的工作原理是为人工智能系统的决策过程提供可解释的见解。 这可能包括显示系统如何做出决策的可视化或对用于达成特定决策的基础流程的解释。

属于分类 https://zhuanlan.zhihu.com/p/589734201


我们是基于大模型的，post hoc interpretation的方法(切记Interpret和explain的异同https://blog.51cto.com/yunyaniu/5677565）。提供一种稳定的热图，同时借助于大模型，实现自动化的语义级别的决策分析。 （我这里大量用了高层语义，语义，这些词可能要慎重使用，我们需要找到支持才能用这些词。因为神经网络浅层是local feature而深层其实是更注重语义的，所以理论上说传统cam在深层channel wise的feature也可以看做语义feature）

原论文中的evaluation contribution我认为没有大的意义，可以删除。



摘要 - 不着急

第一章 - introduction

首页图Teaser的设计 - 一个baseline结果（gradcam）我们的一个属性分析结果+一个融合后的结果



第一段，介绍可解释性工作的重要性。尤其是介绍一下愿景。然后介绍我们希望可解释工作实现的目标。

第二段，介绍已有的可解释性工作，尤其是强调CAM优势和成功应用。我们因此也是希望借用CAM。话锋一转，开始说现在CAM可解释性主要在面临两个问题。第一个问题就是平衡速度和噪声的问题。基于梯度的往往都有更快的速度，但是噪声太大，精度不高。基于遮挡的则往往需要大量反复迭代，速度比较慢。第二个问题就是，现在cam都是在基于channel来分析，也就是所谓的feature-level，来得到热图。最后需要引入人，来进行人为分析。这种所谓的高层语义信息都是通过人的先验，通过人在一个高度复合的热图上进行推断的。比如说，（这里结合teaser，假设是一只猫），说图一这个预测，因为热图集中在猫的头上，所以人们猜测，模型是通过猫头来进行判别这是只猫。但是我们想要强调的是，CAM的热图，(CAM的缺点XXX)。

第三段，开始说我们的方法。通过引入分解+融合这种方式，我们实现了去噪+高层语义级别的分析。进一步我们引入了大模型，最后实现了不需要引入人的分析？（这里在确认下，结合本论文的核心，开始吹）(去噪和高层语义这些最好都需要一些参考文献支持)

第四段，说我们的实验设计，我们有传统的对比，说明噪声去除的比较好，速度和精度保持的也不错。我们有新的属性分析实验，说明了我们的潜力。

最后我们汇总我们的contribution
XX
XX
XX


第二章 - 相关工作
2.1 可解释性工作
第一段，简单介绍下，各种不同的可解释性框架，特别概括，包含gradient，perturbation（occlusion）和CAM。然后话锋一转，说明为啥我们最后借助于cam框架。

第二段，介绍各种cam的主要问题，然后介绍下一些经典cam方法的改进，如gradcam gradcam++ scorecam等等。最后话锋一转，说他们存在什么样的问题。因此我们提出了XXX。


2.2 属性分析
第一段介绍下属性分析以及大模型例如clip等等的重要性。简单的介绍大模型使属性分析进一步成为可能，以及大模型带来的各种可能性。

第二段，分别介绍属性分析、大模型作为可解释性的文章。最后话锋一转，说已有的工作存在的问题。目的是突出我们基于CAM+大模型+属性分析的优点。


第三章 方法
总述，在接下来的章节，我们先介绍我们的基础知识GradCAM，然后我们的Decom-CAM。我们的Decom-CAM分为三个部分，分解（sec.XX），融合（sec.XX），以及一个可选择的属性分析（sec.XX）。
3.1 preliminary - 介绍基础知识GradCAM

3.2 介绍分解过程，原论文中的Decomposition Stage。其中第一段强调svd的motivation - 去噪+成分分析。对应原论文中的图1

3.3 介绍融合过程。原论文中的Integrating Stage。需要一个额外的图，介绍融合过程

3.4 介绍属性分析。需要图包含介绍这部分，可以与3.3的图一起介绍。

3.5 （可选） 可以考虑增加一个3.5，remark，对一些重点问题，如框架、大模型等进行继续的讨论


第四章 实验
总述整体框架的介绍。具体的是4.1介绍啥，4.2介绍啥，接下来，我们在4.3，进行传统任务的的讨论，及不考虑属性分析，只看cam heatmap。在4.4，我们展现我们的框架在新任务上的表现。
4.1 数据集 baseline以及指标的介绍
4.2 部署细节的介绍
4.3 在传统任务的的讨论，包括定位和传统指标的一些任务和可视化
4.4 讨论属性分析，包括可视化以及一些结果展示。最好有一些数据分析，可以考虑调查问卷一类的。






第五章 结论
